OmniLingo: Listening- and speaking-based language learning

In this demo paper we present OmniLingo, an architecture for distributing data for listening- and speaking-based language learning applications and a demonstration client built using the architecture. The architecture is based on the Interplanetary Filesystem (IPFS) and puts at the forefront user sovereignty over data.

==> Makefile <==
all:
	pdflatex omnilingo-nlp4call.tex
	pdflatex omnilingo-nlp4call.tex
	bibtex omnilingo-nlp4call
	pdflatex omnilingo-nlp4call.tex
	pdflatex omnilingo-nlp4call.tex

clean:
	rm -f 	omnilingo-nlp4call.{aux,bbl,blg,log,out,pdf}

ME=$(shell grep "^$$(git config user.email)	" .todomap | cut -f2)
BLAMERS=$(shell cut -f2 .todomap)

todo: todo-$(ME)
	
todo-all:
	@ find * -type f -not -name Makefile -exec grep -Hni '^\s*\(% \)\?TODO\( [^:]*\)\?:' {} \; | awk -F: '{OFS=":"; gsub("^\\s*% ", "", $$3); print}' | sort -t : -k3d,3d -k2n,2n
todo-none:
	@ find * -type f -not -name Makefile -exec grep -Hni '^\s*\(% \)\?TODO:' {} \;
todo-blame:
	@ find * -type f -not -name Makefile -exec grep -i '^\s*\(% \)\?TODO\( [^:]*\)\?:' {} \; | sed -e 's/^\s*\(% \)\?TODO:.*$$//' -e 's/^\s*\(% \)\?TODO \([^:]\+\):.*$$/\2/g' | sort | uniq -c
$(foreach blamer,$(BLAMERS),todo-$(blamer)): todo-%:
	@ find * -type f -not -name Makefile -exec grep -Hni '^\s*\(% \)\?TODO\( $*\)\?:' {} \; | awk -F: '{OFS=":"; gsub("^\\s*% ", "", $$3); print}' | sort -t : -k3d,3d -k2n,2n

